DAGrid: Directed Accumulator Grid

Recent research highlights that the Directed Accumulator (DA), through its parametrization of geometric priors into neural networks, has notably improved the performance of medical image recognition, particularly with small and imbalanced datasets. However, DA's potential in pixel-wise dense predictions is unexplored. To bridge this gap, we present the Directed Accumulator Grid (DAGrid), which allows geometric-preserving filtering in neural networks, thus broadening the scope of DA's applications to include pixel-level dense prediction tasks. DAGrid utilizes homogeneous data types in conjunction with designed sampling grids to construct geometrically transformed representations, retaining intricate geometric information and promoting long-range information propagation within the neural networks. Contrary to its symmetric counterpart, grid sampling, which might lose information in the sampling process, DAGrid aggregates all pixels, ensuring a comprehensive representation in the transformed space. The parallelization of DAGrid on modern GPUs is facilitated using CUDA programming, and also back propagation is enabled for deep neural network training. Empirical results show DAGrid-enhanced neural networks excel in supervised skin lesion segmentation and unsupervised cardiac image registration. Specifically, the network incorporating DAGrid has realized a 70.8% reduction in network parameter size and a 96.8% decrease in FLOPs, while concurrently improving the Dice score for skin lesion segmentation by 1.0% compared to state-of-the-art transformers. Furthermore, it has achieved improvements of 4.4% and 8.2% in the average Dice score and Dice score of the left ventricular mass, respectively, indicating an increase in registration accuracy for cardiac images. The source code is available at https://github.com/tinymilky/DeDA.

==> old_docs/abstract.tex <==
\begin{abstract}


Differentiable Grid Sampling (GS) empowers neural networks to perform spatial transformations previously not possible, enhancing their feature representation capabilities and improving performance across various vision applications.
The Differentiable Directed Accumulator (DA) is a recently developed method that acts as the symmetrical operation to Grid Sampling within the forward-backward deep learning framework. 
This means that the structure of the forward pass of GS is identical to the backward pass of DA.
In this paper, we broaden the application of the existing directed accumulator, originally designed for image classification, to pixel-wise dense mapping applications.

by constructing propose an extension of directed accumulator, that enables neural networks to better preserve or propagate feature information for d.
a new data manipulation operator, the polar accumulator (PA), that enables rotation- and dilation-invariant latent feature representation.
Given a feature map, PA creates and quantizes a polar accumulator space inzto finite intervals based on designated sampling rates, and accumulates feature values accordingly.
Unlike traditional polar transform that the polar representation is sampled from the image representation, PA allows feature aggregation from all pixels in the image space, which means every pixel contributes to the final polar representation.
We parallelize the proposed PA on modern GPUs and enable back propagation for training deep neural networks.
A case study on skin lesion recognition show that the proposed PA can be easily plugged into existing convolutional neural networks and improve recognition performance.
% the value of a cell in PA is the weighted sum of values from all pixels in the feature space that point to the the cell.   




\keywords{Polar accumulator \and Neural networks \and Skin lesion \and Classification}

\end{abstract}

==> old_docs/conclusion.tex <==
\section{Conclusions}








==> old_docs/experiment.tex <==
\section{Experiments and Results}

\subsection{Dataset}

%\subsubsection{ISIC 2018}
The HAM10000 dataset~\cite{tschandl2018ham10000} was used as the training dataset for the ISIC 2018 skin lesion classification challenge\footnote{https://challenge.isic-archive.com/data/\#2018}. It comprises of 10,015 skin lesion images that fall under seven types of skin lesions, which include malignant melanoma (MEL), melanocytic nevus (NV), basal cell carcinoma (BCC), actinic keratosis/bowen’s diseases (AK), benign keratosis-like lesion (BKL), dermatofibroma (DF) and vascular (VASC).

%\subsubsection{ISIC 2019}
%The ISIC 2019 dataset\footnote{https://challenge.isic-archive.com/data/\#2019} is a combination of three datasets, namely the HAM dataset~\cite{tschandl2018ham10000}, MSK dataset~\cite{codella2018skin}, and BCN\_20000 dataset~\cite{combalia2019bcn20000}. It includes a total of 25,331 images belonging to eight categories of skin lesions, namely MEL, NV, BCC, AK, BKL, DF, VASC, and squamous cell carcinoma (SCC). 


\subsection{Baseline and Implementation}








\subsection{Classification Performance}

\begin{table}[!t]
\caption{Skin lesion classification performance on the independent test set. The left panel shows the standard-data regime (70\% training) and the right panel shows the low-data regime (20\% training). The best performing metric is bolded.
}
\vspace{-1ex}
\label{tab:overall}
%\vskip 0.15in
\begin{center}
\resizebox{1.\columnwidth}{!}{
%\setlength{\tabcolsep}{4pt}
\begin{tabular}{ lccccc| lccccc}
\hline
\hline
\multicolumn{6}{c|}{\underline{70\% (Train) : 10\% (Val) : 20\% (Test)}} & \multicolumn{6}{c}{\underline{20\% (Train) : 10\% (Val) : 70\% (Test)}} \\
Model	&Accuracy &$F_1$ 	&Sensitivity	&Specificity	&AUC & Model &Accuracy &$F_1$ 	&Sensitivity	&Specificity	&AUC \\
\hline
ResNet-18 & 0.797 &	0.606 & 0.634	& 0.587	& 0.938 & ResNet-18 & 0.751 &	0.513 &	0.561 &	0.489 &	0.885 \\
ResNet-34 & 0.802 &	0.623 &	0.645 &	0.614 &	0.927 &  ResNet-34 & 0.743 &	0.488 &	0.530 &	0.475 &	0.884 \\
ResNet-50 & 0.791 &	0.592 &	0.623 &	0.585 &	0.933 & ResNet-50 & 0.721 &	0.437 &	0.442 &	0.434 &	0.884 \\
ResNet-101 & 0.760 & 0.479 & 0.532 & 0.459 & 0.910 & ResNet-101 & 0.727 & 0.415 & 0.426 & 0.408 & 0.880 \\
\hline
DenseNet-121 & 0.802 & 0.652 &	0.676 &	0.631 &	0.927 & DenseNet-121 & 0.744 &	0.468 &	0.511 &	0.443 &	0.881 \\
DenseNet-161 & 0.802 &	0.648 &	0.669 &	0.635 &	0.936 & DenseNet-161 & 0.727 &	0.461 &	0.480 &	0.453 &	0.884 \\
DenseNet-169 & 0.800 &	0.652 &	0.662 &	0.644 &	0.915 & DenseNet-169 & 0.750 &	0.480 &	0.517 &	0.460 &	0.879 \\
DenseNet-201 & 0.785 &	0.548 &	0.649 &	0.494 &	0.926 & DenseNet-201 & 0.718 &	0.437 &	0.454 &	0.436 &	0.882 \\
\hline
Swin-T & 0.734 & 0.464 & 0.460 & 0.474 & 0.918 & Swin-T & 0.713 & 0.416 & 0.506 & 0.396 & 0.896 \\
Swin-S & 0.746 & 0.489 & 0.543 & 0.484 & 0.916 & Swin-S & 0.733 & 0.485 & 0.521 & 0.468 & 0.898 \\
Swin-B & 0.753 & 0.479 & 0.631 & 0.461 & 0.924 & Swin-B & 0.682 & 0.379 & 0.369 & 0.431 & 0.877 \\
\hline
ResNet-PA-1281 & 0.791 & 0.604 & 0.619 & 0.594 & 0.937 & ResNet-PA-1281  & 0.749 & 0.486 &	0.507 &	0.492 &	\bf{0.908} \\
ResNet-PA-2562  & 0.815 & 0.638 & 0.660 & 0.629 & \bf{0.950} & ResNet-PA-2562  & 0.757 &	0.507 &	\bf{0.566} &	0.499 &	\bf{0.908} \\
\hline
DenseNet-PA-1281 & 0.807 &	0.646 &	0.691 &	0.620 &	0.937 & DenseNet-PA-1281  & \bf{0.759} &	\bf{0.515} &	0.563 &	\bf{0.502} &	0.894 \\
DenseNet-PA-2562  & \bf{0.820} &	\bf{0.677} &	\bf{0.712} &	\bf{0.652} &	0.946 & DenseNet-PA-2562  &  0.758 &	0.498	& 0.547 &	0.481 &	\bf{0.908} \\
\hline
\hline
\end{tabular}
}
\end{center}
\vspace{-1ex}
\end{table}








\subsection{Ablation Study on }


\begin{table}[!t]
\caption{Ablation study on . The left panel shows the standard-data regime (70\% training) and the right panel shows the low-data regime (20\% training). The best performing metric is bolded.
}
\vspace{-1ex}
\label{tab:overall}
%\vskip 0.15in
\begin{center}
\resizebox{1.\columnwidth}{!}{
%\setlength{\tabcolsep}{4pt}
\begin{tabular}{ lccccc| lccccc}
\hline
\hline
\multicolumn{6}{c|}{\underline{70\% (Train) : 10\% (Val) : 20\% (Test)}} & \multicolumn{6}{c}{\underline{20\% (Train) : 10\% (Val) : 70\% (Test)}} \\
Model	&Accuracy &$F_1$ 	&Sensitivity	&Specificity	&AUC & Model &Accuracy &$F_1$ 	&Sensitivity	&Specificity	&AUC \\
\hline
PA-641 &  0.768 &	0.543 &	0.609 &	0.559 &	0.928  \\
PA-642 &  0.803 &	0.602 &	0.631 &	0.582 &	0.938  \\
PA-644 &  0.793 &	0.582 &	0.635 &	0.556 &	0.930  \\
\hline
PA-1281 & 0.791 &	0.604 &	0.619 &	0.594 &	0.937 & PA-1281 & 0.749 &	0.486 &	0.507 &	0.492 &	0.908 \\
PA-1282 & 0.804 &	0.620 &	0.643 &	0.645 & 0.940 & PA-1282 & 0.714 &	0.437 &	0.476 &	0.441 &	0.902 \\
PA-1284 & 0.800 &	0.586 &	\bf{0.725} &	0.565 &	0.936 \\
\hline
PA-2561 & 0.806 &	0.660 &	0.683 &	0.643 &	0.933 & PA-2561 & \bf{0.759} &	0.505 &	0.546 &	0.491 &	\bf{0.909} \\
PA-2562 & 0.815 &	0.638 &	0.660 &	0.629 &	\bf{0.950} & PA-2562 & 0.757 &	\bf{0.507} &	\bf{0.566} &	\bf{0.499} &	0.908 \\
PA-2564 & 0.802 &	0.623 &	0.655 &	0.602 &	0.937  \\
\hline
PA-5121 & 0.814 &	\bf{0.681} &	0.693 &	\bf{0.675} &	0.947  \\
PA-5122 & \bf{0.817} &	0.674 &	0.709 &	0.659 &	0.946  \\
\hline
\hline
\end{tabular}
}
\end{center}
\vspace{-1ex}
\end{table}



==> old_docs/introduction.tex <==
\section{Introduction}

Skin cancer is one of the most common malignancies in the world, with incidence significantly increasing over the past decade~\cite{vestergaard2008dermoscopy}. 
Typically, dermatologists diagnose skin cancer based on visual inspections, supported by dermoscopic imaging and skin biopsy confirmation~\cite{vestergaard2008dermoscopy}. 
However, rural communities often lack access to prompt skin cancer detection due to a shortage of dermatologists and pathology lab facilities. 
This can lead to increased morbidity and melanoma mortality rates~\cite{feng2018comparison}.
By applying machine learning techniques to skin lesion classification, we can potentially automate the screening and early detection of skin cancer.
Previous approaches for computer-aided dermoscopic image analysis relied on extracting handcrafted features and inputting them into conventional classifiers~\cite{yang2018clinical}. 
Recent advancements in automatic skin cancer classification have significantly improved performance by utilizing end-to-end training of deep convolutional neural networks~\cite{esteva2017dermatologist, liu2020deep}.

Publicly accessible datasets for skin lesions usually lack sufficient sample sizes, especially in cases where the lesions have low contrast, fuzzy borders, and other interferences~\cite{tschandl2018ham10000, codella2018skin}. 
In order to train a neural network to fit unknown data features, a sufficient sample size is necessary - this is exemplified by the tens of millions of data used for algorithm performance verification in the commonly used ImageNet~\cite{deng2009imagenet}. 
While previous deep learning models have achieved significant diagnostic outcomes comparable to professional dermatologists, most of the training datasets for these models are derived from private datasets that are not publicly accessible~\cite{esteva2017dermatologist, liu2020deep}.
In contrast, publicly available dermoscopic image datasets generally have only a few thousand samples~\cite{tschandl2018ham10000, codella2018skin}.

Recently, a lot of efforts have been focusing on designing neural network architectures where domain-specific (prior) knowledge is injected, in order to improve image analysis robustness when image artifacts are significant and sample size is limited~\cite{oktay2017anatomically, seo2019modified, clough2020topological, xie2021survey}.
One stream of the work benefits from learning high-level object features~\cite{oktay2017anatomically, seo2019modified}.
For example, an autoencoder is used to extract global anatomical shape properties, which regularizes the cardiac segmentation framework to incorporate the prior structural information~\cite{oktay2017anatomically}.
On the other hand, some work are inspired by the topological signal processing properties~\cite{clough2020topological}.
For instance, deep directed accumulator, a symmetric operator, is proposed to transform images from discrete space to functional space where geometric information is better aggregated for multiple sclerosis lesions diagnosis. 

In this work, we tackle the large intra-class variations and small sample size problems of skin lesion classification by incorporating the lesions' geometric information via polar transformation.
Polar transform, a signal processing approach, has been widely used in computer vision tasks~\cite{esteves2017polar, xie2020polarmask, park2022eigencontours}.
It has two intriguing properties: 1) polar transformation preserves the shape information of the target~\cite{xie2020polarmask, park2022eigencontours}; 2) its representation is rotationally equivariant from the nature of polar coordinate system~\cite{esteves2017polar}.
Inspired by the deep directed accumulator, we project discrete signals from image space to polar coordinates using the differentiable directed accumulation technique.
This is a symmetric operation to the grid sampling~\cite{jaderberg2015spatial} that enables us to perform the polar transformation within a forward-backward learning framework.
We evaluate our proposed medthod on the public skin lesion dataset ISIC 2018~\cite{tschandl2018ham10000}.



==> old_docs/method.tex <==
\section{Methodology}

The polar accumulator (PA) is inspired by a recently proposed image transformation operator deep directed accumulator (DeDA).
We will briefly review DeDA and dervie the proposed PA.

\subsection{Preliminaries on DeDA}

Given a source feature map $\mathbf{U} \in \mathbb{R}^{C\times H \times W}$, a target feature map $\mathbf{V} \in \mathbb{R}^{C\times H' \times W'}$, a set of sampling grids $\mathcal{G} = \{\mathbf{G}[k] \in \mathbb{R}^{2\times H \times W}=(\mathbf{G}^x[k], \mathbf{G}^y[k])~|~k \in \mathbb{Z}^+, 1 \leq k \leq N \}$ ($N\geq 1$ is the number of grids), and a kernel function $\mathcal{K}()$, the output value of a particular position $(i,j)$ at the target feature map $\mathbf{V}$ can be written as follows:
\begin{equation}
    \mathbf{V}_{ij}^{c} = \sum_k^{N}\sum_n^{H}\sum_m^{W} \mathbf{U}_{nm}^{c}\mathcal{K}(\mathbf{G}_{nm}^x[k],i)\mathcal{K}(\mathbf{G}_{nm}^y[k],j),
    \label{eq:deda}
\end{equation}
where the kernel function $\mathcal{K}()$ can be replaced with any other specified kernels, e.g. integer sampling kernel $\delta(\lfloor\mathbf{G}_{nm}^x+0.5\rfloor-i)\cdot \delta(\lfloor\mathbf{G}_{nm}^y+0.5\rfloor-j)$ and bilinear sampling kernel $\text{max}(0,1-|\mathbf{G}_{nm}^x-i|) \cdot \text{max}(0,1-|\mathbf{G}_{nm}^y-j|)$. 
Here $\lfloor x+0.5\rfloor$ rounds $x$ to the nearest integer and $\delta()$ is the Kronecker delta function.
The gradients with respect to $\mathbf{U}$ for back propagation can be defined accordingly \cite{deda}.

The structure of Eq.~\ref{eq:deda} is similar to spatial grid sampling; however, as mentioned in \cite{deda}, DeDA is  symmetric to the grid sampling, enabling easy integration of geometric prior such as line and rim parameterization along with long-range contextual information into deep neural networks.

\subsection{Differentiable Deep Polar Accumulator}

We introduce the proposed PA in the context of the forward-backward deep learning framework and name it as deep polar accumulator (DePA).
The DePA mainly consists of three components: 1) polar grid creation by value accumulation, 2) polar grid processing, and 3) extraction of feature map by slicing the polar grid.

\subsubsection{Polar Grid Definition and Creation.}

The polar grid is a three dimensional tensor, where the first dimension $c$ corresponds to the feature channels such as RGB values, while the last two dimensions $(r,\psi)$ correspond to a 2D position in the polar plane and form the spatial domain.
A polar grid $\mathbf{P} \in \mathbb{R}^{C\times N_{r} \times W_{\psi}}$ is regularly accumulated in the spatial dimension from a given feature map $\mathbf{U} \in \mathbb{R}^{C\times H\times W}$ and each channel $c$ is transformed in an identical way.
To map from feature map $\mathbf{U}$ to polar grid $\mathbf{P}$ using Eq.~\ref{eq:deda}, we need to define the sampling grid set $\mathcal{G}$.
Let the mesh grids of $\mathbf{U}$ be $\mathbf{M}^x \in \mathbb{R}^{H\times W}$ (value range: $(0,H-1)$) and $\mathbf{M}^y \in \mathbb{R}^{H\times W}$ (value range: $(0,W-1)$), the coordinate of image center be $(x_c,y_c)$, the value of sampling grid along $x$ direction $\mathbf{G}^{x}$ at position $(i,j)$ can be obtained as follows:
\begin{equation}
    \mathbf{G}^{x}_{ij} = \sqrt{(\mathbf{M}^x_{ij} - x_c)^2 + (\mathbf{M}^y_{ij} - y_c)^2} / s_r, 
\end{equation}
where $s_r$ is the sampling rate along the radial direction.
Similarly, the value of sampling grid along $y$ direction $\mathbf{G}^{y}$ at position $(i,j)$ can be obtained as follows:
\begin{equation}
    \mathbf{G}^{y}_{ij} = \arctan{((\mathbf{M}^x_{ij} - x_c)^2 + (\mathbf{M}^y_{ij} - y_c)^2} + \pi) / s_{\theta}, 
\end{equation}
where $s_{\theta}$ is the sampling rate along the angular direction, and $+\pi$ is used to pull all values to the range of $(0,2\pi)$.
Now the value at position $(i,j)$ channel $c$ of polar grid $\mathbf{P}$ can be defined as follows:
\begin{equation}
    \mathbf{P}_{ij}^{c} = \sum_n^{H_r}\sum_m^{W_{\psi}} \mathbf{U}_{nm}^{c}\text{max}(0,1 - |\mathbf{G}_{nm}^x[k]-i|)\text{max}(0, 1- |\mathbf{G}_{nm}^y[k]-j|),
    \label{eq:depa}
\end{equation}

\subsubsection{Homogeneous Values.}

As denoted in Eq.~\ref{eq:depa}, the value of each cell in the polar grid is the weighted sum of values from cells in the feature map. 
To keep track of the number of pixel values (or a weight tensor $\mathbf{W}$) that correspond to the polar grid cell, we store homogeneous quantities as $(\mathbf{P}_{ij}^{c},\mathbf{W}_{ij})$.
Since $\mathbf{W}$ expands only two dimensions, in practice, $\mathbf{W}$ and $\mathbf{P}$ can be stored separately.
Similarly using Eq.~\ref{eq:deda}, we can define the value at position $(i,j)$ of $\mathbf{W}$ as follows:
\begin{equation}
    \mathbf{W}_{ij} = 1/(\sum_n^{H_r}\sum_m^{W_{\psi}} \text{max}(0,1 - |\mathbf{G}_{nm}^x[k]-i|)\cdot\text{max}(0, 1- |\mathbf{G}_{nm}^y[k]-j|)+\epsilon),
    \label{eq:depa}
\end{equation}
where $\epsilon$ is a small real value to avoid zero denominator.

\subsubsection{Polar Grid Processing and Slicing.}


